Formal Modeling and SMT-Based Parameterized Verification of Multi-Case Data-Aware BPMN

We propose DAB -- a data-aware extension of the BPMN de-facto standard with the ability of operating over case and persistent data (partitioned into a read-only catalog and a read-write repository), and that balances between expressiveness and the possibility of supporting parameterized verification of safety properties on top of it. In particular, we take inspiration from the literature on verification of artifact systems, and consider verification problems where safety properties are checked irrespectively of the content of the read-only catalog, possibly considering an unbounded number of active cases and tuples in the catalog and repository. Such problems are tackled using fully implemented array-based backward reachability techniques belonging to the well-established tradition of SMT model checking. We also identify relevant classes of DABs for which the backward reachability procedure implemented in the MCMT array-based model checker is sound and complete, and then further strengthen such classes to ensure termination.

==> app-7-experiments.tex <==
\section{Experiments}
\label{app_experiments}

\begin{table}
  \centering
  \caption{Summary of the experimental examples}
  \label{tab:benchmark}
        \begin{tabular}{llrrr}\toprule
       \multicolumn{2}{l}{\textbf{Example}} & \textbf{\#AC} & \textbf{\#AV} &\textbf{\#T} \\\midrule
            E1& JobHiring &9 & 18 & 15\\
            E2& Acquisition-following-RFQ &6 &13 &28\\
            E3& Book-Writing-and-Publishing & 4 & 14 & 13\\
            E4& Customer-Quotation-Request & 9 & 11 & 21\\
            E5& Patient-Treatment-Collaboration & 6 & 17 & 34\\
            E6& Property-and-Casualty-Insurance-Claim-Processing & 2 & 7 &15\\
            E7& Amazon-Fulfillment &  2 & 28 & 38\\
            E8& Incident-Management-as-Collaboration & 3 & 20 & 19
            \\\bottomrule
        \end{tabular}
    \end{table}



We base our experimental evaluation on the already existing benchmark provided in \cite{verifas}, that samples 32 real-world BPMN workflows published at the official BPM website (\url{http://www.bpmn.org/}).
Specifically, inspired by the specification approach adopted by the authors of \cite{verifas} in their experimental setup (\url{https://github.com/oi02lyl/has-verifier}), we select seven examples of varying complexity (see Table~\ref{tab:benchmark}) and provide their faithful encoding\footnote{Our encoding considers semantics of the framework studied in \cite{verifas}.} in the array-based specification using MCMT Version~2.8 (\url{http://users.mat.unimi.it/users/ghilardi/mcmt/}). Moreover, we enrich our experimental set with an extended version of the running example from Appendix~\ref{sec:hiring-example}. Each example has been checked against at least one safe and one unsafe conditions.
Experiments were performed on a machine with Ubuntu~16.04, 2.6\,GHz Intel
Core~i7 and 16\,GB RAM.


%The time limit for each example has been empirically set to 7200sec: this time suffices to generate relatively big transition systems and recognize growth patterns in the conducted experiments.



\begin{table}
  \centering
  \caption{Experimental results for safety properties}
  \label{tab:exp_extended}
        \begin{tabular}{cccrrrr}\toprule
            \textbf{Example} & \textbf{Property}&\textbf{Result}&\textbf{Time} &\textbf{\#N}  & \textbf{depth} &\textbf{\#SMT-calls}
            \\\midrule
            E1& E1P1 & \safe & 0.06 & 3 &  3 & 1238\\
             & E1P2& \unsafe & 0.36 & 46 & 10 & 2371\\
             & E1P3 & \unsafe &0.50 & 62 & 11 & 2867 \\
              & E1P4 & \unsafe & 0.35 & 42 & 10 & 2237 \\
            E2 & E2P1&  \safe & 0.72 & 50 & 9 & 3156\\
              & E2P2 &  \unsafe & 0.88 & 87 & 10 & 4238\\
              & E2P3& \unsafe &1.01 & 92 & 9 & 4811\\
             & E2P4 &  \unsafe & 0.83  & 80 & 9 & 4254\\
            E3 &  E3P1&  \safe & 0.05 & 1 & 1 & 700\\
             &E3P2 &  \unsafe & 0.06 & 14 & 3 & 899\\
            E4  & E4P1&  \safe &0.12 & 14 & 6 & 1460\\
              & E4P2&  \unsafe & 0.13 & 18 & 8 & 1525\\
           E5  & E5P1&  \safe &4.11 & 57 & 9 & 5618\\
              & E5P2&  \unsafe & 0.17& 13 & 3 & 2806\\
            E6   & E6P1& \safe & 0.04& 7 & 4 & 512\\
               & E6P2&  \unsafe &0.08 & 28 & 10 & 902\\
            E7  & E7P1 &  \safe & 1.00& 43 & 7 & 5281\\
             & E7P2&  \unsafe & 0.20 & 7 & 4 & 3412\\
            E8  & E8P1&  \safe & 0.70& 77 & 11 & 3720\\
              & E8P2 &  \unsafe & 0.15 & 25 & 7 & 1652
            \\\bottomrule
        \end{tabular}
\end{table}

%    \begin{table}\centering
%        \begin{tabular}{cccccccccccccccccccc}\toprule
%       \rotatebox{90}{Acquisition-following-RFQ\_1.txt}
%            & \rotatebox{90}{Acquisition-following-RFQ\_2.txt}
%            & \rotatebox{90}{Acquisition-following-RFQ\_3.txt}
%            & \rotatebox{90}{Acquisition-following-RFQ\_4.txt}
%            & \rotatebox{90}{JobHiring\_1.txt}
%            & \rotatebox{90}{JobHiring\_2.txt}
%            & \rotatebox{90}{JobHiring\_3.txt}
%            & \rotatebox{90}{JobHiring\_4.txt}
%            & \rotatebox{90}{Book-Writing-and-Publishing\_1.txt}
%            & \rotatebox{90}{Book-Writing-and-Publishing\_2.txt}
%            & \rotatebox{90}{Customer-Quotation-Request\_1.txt}
%            & \rotatebox{90}{Customer-Quotation-Request\_2.txt}
%            & \rotatebox{90}{Patient-Treatment-Collaboration\_1.txt}
%            & \rotatebox{90}{Patient-Treatment-Collaboration\_2.txt}
%            & \rotatebox{90}{Property-and-Casualty-Insurance-Claim-Processing\_1.txt}
%            & \rotatebox{90}{Property-and-Casualty-Insurance-Claim-Processing\_2.txt}
%            & \rotatebox{90}{Amazon-Fulfillment\_1.txt}
%            & \rotatebox{90}{Amazon-Fulfillment\_2.txt}
%            & \rotatebox{90}{Incident-Management-as-Collaboration\_1.txt}
%            & \rotatebox{90}{Incident-Management-as-Collaboration\_2.txt}
%
%            \\\bottomrule
%        \end{tabular}
%        \caption{Experimental results for safety properties}\label{tab:exp_extended}
%    \end{table}





Here \textbf{\#AV}, \textbf{\#AC} and \textbf{\#T} represent, respectively, the number of artifact variables, artifact components and transitions used in the example specification, while \textbf{Time} is the \mcmt execution time. The most critical measures are \textbf{\#N}, \textbf{depth} and \textbf{\#SMT-calls} that respectively define the number of nodes and the depth of the tree used for the backward reachability procedure adopted by \mcmt, and the number of the SMT-solver calls.
 Indeed, \mcmt  computes the iterated preimages of the formula describing the unsafe states along the various transitions. Such computation produces a tree, whose nodes are labelled by formulae describing sets of states that can reach an unsafe state and whose arcs are labelled by a transition.
In other words, an arc $t:\phi \rightarrow \psi$ means that $\phi$ is equal to $Pre(t,\psi)$. The tool applies forward and backward simplification strategies, so that whenever a node $\phi$ is deleted, this means that $\phi$ entails the disjunction of the remaining (non deleted) nodes. All nodes (both deleted and undeleted) can be visualized via the available online options (it is also possible to produce a Latex file containing their detailed description)


To stress test our encoding, we came up with a few formulae describing unsafe configurations (sets of ``bad'' states), that is, the configurations that the system should not incur throughout its execution.
%(un)safe conditions that stay in line with specific semantics of the chosen examples.
%Table~\ref{tab:exp_extended} considers formulae defining properties that the examples in Table~\ref{tab:benchmark} are checked against.
%These formulae describe unsafe configurations (sets of ``bad'' states), that is, the configurations that the system should not incur throughout its execution.
\textbf{Property} references encodings of examples endowed with specific (un)safety properties done in \mcmt, whereas \textbf{Result} shows their verification outcome that can be of the two following types: \safe and \unsafe.
The \mcmt tool returns \safe, if the undesirable property it was asked to verify represents a configuration that the system cannot reach.
At the same time, the result is \unsafe  if there exists a path of the system execution that reaches ``bad'' states.
One can see, for example, that the job hiring \ras has been proved by \mcmt to be \safe w.r.t. the property defined in Example~\ref{ex:hr-prop}. The details about the successfully completed verification task can be seen in the first row of Table~\ref{tab:exp_extended}: the tool constructed a tree with 3 nodes and a depth of 3, and returned \safe in 0.06 seconds.
For the same job hiring \ras, if we slightly modify the safe condition discussed in Example~\ref{ex:hr-prop} by removing, for instance,
the check that a selected applicant is not a winning one, we obtain a description (see below) of a configuration in which it is still the case that an applicant could win:
\[
  \begin{array}{@{}l@{}}
   \exists  \typedvar{i}{\appidx}
    \left(  \begin{array}{@{}l@{}} \pstatev=\notified \land \appuser[i]\neq \nullv
    {}\land  \appres[i]\neq \los
    \end{array}
    \right)
  \end{array}
\]
In this case, the job hiring process analyzed against the devised property is evaluated as \unsafe by the tool (see E1P3 row in Table~\ref{tab:exp_extended}). When checking safety properties, \mcmt also allows to access an unsafe path of a given example in case
the verification result is \unsafe.


To conclude, we would like to point out that seemingly high number of SMT solver calls in \textbf{\#SMT-calls} against relatively
small execution time demonstrates that \mcmt could be considered as a promising tool supporting the presented line of research.
This is due to the following two reasons. On the one hand, the SMT technology underlying  solvers like \textsc{Yices} \cite{Dutertre} is quite mature and impressively well-performing. On the other hand, the backward reachability algorithm generates proof obligations which are relatively easy
to be analyzed as (un)satisfiable by the solver.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Specifically, we consider the Acquisition-following-RFQ example that models an acquisition process following request for quotation from selected suppliers.
In this process, a customer may request goods from a supplier.
If no supplier is found or the contacted supplier could not fulfill the request, the process sends a notice to
the customer and changes its global status to \emph{NoticeSent}.
Otherwise, the process computes the optimal quote and, if the customer agrees on it, sends the requested goods to her and changes its global status to \emph{Acquired}.
This completes one of the possible process executions.
In our model, the global status is represented using a global artifact variable.
However, according to semantics adopted in the original benchmark, artifact variables, if not being propagated, may non-deterministically acquire values.

Hence, we exclude

Let us now to use this execution example so to generate an unsafe conditions to check.
Semantics of the models from \cite{verifas} allows to ``generate'' any kind of values in the variables


To represent the global status, we use in our MCMT encoding a global artifact variable that, however, may change its value regardless t



 In both of these situations, the artifact variables different from "Status" are meaningless: so, this is the only case when the supplier provides answer yes with a customer that does not exist ("null"). Hence, if status is different from "Acquired" and . This is our unsafe condition, and the tool returns that this system is SAFE, i.e. it is not possible to reach the configuration when a customer is null and the response of the supplier is affermative (unless status has those specific values). If we delete the restrictions over the values of status, the system is detected by the tool to be UNSAFE, as expected: in fact, starting from the initial condition, it is possible to reach the unwanted  configuration due to presence of the non-deterministic reassignement of values of the artifact variables in the case the only relevant variable is the one describing the status.

 The remaining 4 cannot be expressed
in HAS* because they involve computing aggregate functions or updating
unboundedly many tuples of the artifact relations, which is
not supported in the current model.

\textbf{DO WE HAVE OPTIMIZATIONS?}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> bpmn-example.tex <==


\begin{figure}[t!]
\hspace*{-1.3cm}
\resizebox{1.2\textwidth}{!}{
\begin{tikzpicture}[auto,x=1.4cm,y=.9cm, thick,minimum size=.8cm]

%applicant lane
%\node[draw,rectangle,rounded corners,minimum width = 12.2cm,minimum height=.9cm] (applicant) at (6.6,2) {Applicant} ;
%subprocess block
\node[draw,rectangle,rounded corners,minimum width = 12.2cm,minimum height=4.7cm] (spb) at (6.6,-1.6) {} ;


\node[MessageStartEvent] (jobe) at (1.5,0) {};
\node[lbl,below of=jobe,align = center] (jobe_name) {Job posted\\ $\left[\updatespec{InsJobCat}\right]$\\~};
\draw[sequence,->]  (jobe) -- (2.28,0);


\node[StartEvent] (se1) at (2.7,0) {};
\node[lbl,below of=se1,align = center] (se1_name) {};
\node[ExclusiveGateway,draw] (eg1) at (3.7,0) {};
\draw[sequence,->]  (se1) -- (eg1);

\node[EventBasedGateway,draw] (eg_err) at (4.8,0) {};
\node[draw,regular polygon,regular polygon sides=5,minimum width=1mm,scale=0.35] at (4.8,0){};
\draw[sequence,->]  (eg1) -- (eg_err);


\node[MessageIntermediateCatchingEvent] (appe) at (6,0) {};
\node[lbl ,below of=appe,align = center,yshift=1mm] (appe_name) {App.~received\\$\left[\updatespec{InsUser}\right]$};
\draw[sequence,->]  (eg_err) -- 
%node[guard,xshift=-2mm,yshift=-.3cm,align=left] {$tPassed=$\\\constant{'1 month'}}  
(appe);


\node[MessageIntermediateCatchingEvent,draw,minimum size=.8cm] (msg-exp) at (6,-2.2) {};
\node[lbl ,below of=msg-exp,align = center,yshift=1mm] (msg-exp_name) {Stop\\~};
\draw[sequence,rounded corners=5pt,->] (eg_err) |- 
%node[guard,xshift=0mm,yshift=5mm,align=left] {$tPassed\neq$\\\constant{'1 month'}} 
(msg-exp);

\node[ErrorEndEvent,draw,minimum size=.8cm] (err) at (7.3,-2.2) {};
\node[lbl ,below of=err,align = center,yshift=1mm] (msg-exp_name) {Stopped\\~};
\draw[sequence,rounded corners=5pt,->] (msg-exp)--(err);

%node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] (c) at (6,1.5) {};
%\draw[sequence,dashed,->]  (c) -- (appe);







\node[task,align=center] (evalcv) at (7.3,0) {\tname{Evaluate}\\\tname{CV}};
\node[lbl ,below of=evalcv,align = center,yshift=1mm] {$\left[\updatespec{CheckQual}\right]$};
\draw[sequence,->]  (appe) -- (evalcv);

\node[ExclusiveGateway,draw] (eg2) at (8.6,0) {};
\draw[sequence,->]  (evalcv) -- (eg2);

\node[EndEvent] (ee1) at (10.5,0) {};
\node[lbl,below of=ee1,align = center] (ee1_name) {};
\draw[sequence,->]  (eg2) -- node[below,align=left] {$\cvar{qualif}=$\\\true} (ee1);


\node[task,align=center] (evalapp) at (8.6,-3.3) {\tname{Evaluate}\\\tname{Application}};
\node[lbl ,right of=evalapp,anchor=west,align = left] {$\left[\updatespec{EvalApp}\right]$};
\draw[sequence,->,rounded corners=5pt] (eg2) -- node[guard,align=left] {$\cvar{qualif}=$\\\false} (evalapp);
\draw[sequence,->,rounded corners=5pt] (evalapp) -| (eg1);



\node[ErrorIntermediateEvent,fill=white] (eb) at (10.95,-3.5) {};
\node[lbl,below right of=eb,align = center,xshift=-.05cm] (eb_name) {Stopped};

\node[task,align=center] (eligcand) at (13.3,-3.5) {\tname{Decide}\\\tname{Eligible}\\\tname{Candidates}};
\node[lbl ,right of=eligcand,anchor=west,align = left] {$\left[\updatespec{MarkE}\right]$};
\draw[sequence,->,rounded corners=5pt] (eb) -- (eligcand);

%
%\node[ExclusiveGateway,draw] (eg_elig) at (12,-5.3) {};
%\draw[sequence,->]  (eligcand) --  (eg_elig);
%

\node[task,align=center] (dwinner) at (13.3,-1.6) {\tname{Select}\\\tname{Winner}};
\node[lbl ,right of=dwinner,anchor=west,align = left] {$\left[\updatespec{SelWinner}\right]$};
\draw[sequence,->]  (eligcand) --  (dwinner);


%
%\draw[sequence,->,rounded corners=5pt]  (eg_elig) -- node[guard,xshift=1.3cm,yshift=-.1cm,align=left] {$exists\_eligible=$\\\true}  (dwinner);
%
\node[task,align=center] (awinner) at (12,0) {\tname{Assign}\\\tname{Winner}};
\draw[sequence,->,rounded corners=5pt] (10.93,0) -- (awinner);


\node[ExclusiveGateway,draw] (eg3) at (13.3,0) {};
\draw[sequence,->]  (awinner) --  (eg3);
\draw[sequence,->]  (dwinner) --  (eg3);

\node[task,align=center] (offer) at (14.5,0) {\tname{Make}\\\tname{Offer}};
\draw[sequence,->]  (eg3) --  (offer);


\node[EndEvent] (ee2) at (15.9,0) {};
\node[lbl,below of=ee2,align = center] (ee2_name) {};
\draw[sequence,->]  (offer) --  (ee2);


%\node[EndEvent] (ee3) at (15.9,-5.3) {};
%\node[lbl,below of=ee2,align = center] (ee2_name) {};
%\draw[sequence,->]  (eg_elig) --  node[guard,xshift=-.2cm,yshift=-.3cm,align=left] {$exists\_eligible=$\\\false} (ee3);
\end{tikzpicture}
}
\caption{The job hiring process. Elements in squared brackets indicate the update specifications attached to the corresponding tasks/events, and formalized as shown in Examples~\ref{ex:updates-1} and~\ref{ex:updates-2}.}
\label{fig:bpmn-hiring}
\end{figure}

==> mcmt.tex <==
\section{First Experiments with MCMT}
\label{sec:mcmt}
We have manually encoded the job hiring \dab described in the paper as an \mcmt specification, using the same translation rules recalled in Section~\ref{sec:translation} and fully spelled out in the Appendix towards proving the main theorems in Sections~\ref{sec:soundness-completeness} and \ref{sec:termination}. \textsc{mcmt} 
checks unsafety of a property through a symbolic, backward reachability procedure. 
The algorithm computes iterated preimages of the given property and applies to
them quantifier elimination, until a fixpoint is reached or until a set
intersecting the initial state (i.e., also characterized using a formula) is found. To do this efficiently, \mcmt is equipped with dedicated quantifier elimination techniques, and discharge safety and fixpoint tests encountered during the backward search to state-of-the-art SMT solvers.



%
%
%
%
% \begin{wrapfigure}[14]{r}{0.45\textwidth}
% \vspace{-22pt}
% \small
%\begin{algorithm}[H]
%\SetKwProg{Fn}{Function}{}{end}
%\Fn{$\mathsf{BReach}(\upsilon)$}{
%\setcounter{AlgoLine}{0}
%\ShowLn$\phi\longleftarrow \upsilon$;  $B\longleftarrow \bot$\;
%\ShowLn\While{$\phi\land \neg B$ is $T$-satisfiable}{
%\ShowLn\If{$\iota\land \phi$ is $T$-satisfiable.}
%{\textbf{return}  $\mathsf{unsafe}$}
%\setcounter{AlgoLine}{3}
%\ShowLn$B\longleftarrow \phi\vee B$\;
%\ShowLn$\phi\longleftarrow \mathit{Pre}(\tau, \phi)$\;
%\ShowLn$\phi\longleftarrow \mathsf{QE}(T^*,\phi)$\;
%}
%\textbf{return} $(\mathsf{safe}, B)$;}{
%\caption{Backward reachability algorithm}\label{alg1}
%}
%\end{algorithm}
% \end{wrapfigure}
% 
% In order to assess safety property over DABs, we exploit a translation of DABs into RASs, a formalism presented in~\cite{CGGMR18,CGGMR19}. To attack the verification of RASs, we implemented a prototype of the \emph{backward reachability algorithm} on top of the \textsc{mcmt} model checker for array-based systems.
% \textsc{mcmt} manages infinite-state verification by exploiting
% as its model-theoretic framework the declarative formalism of array-based
% systems.  This formalism allows for symbolic representation of transitions
% and sets of states using formulae, whereas the system dynamics is defined by
% manipulating function  variables (i.e., arrays).
%%
%% \textsc{mcmt}, in turn, is capable of verifying (safety) properties of a
%% large class of infinite state systems which are specified using the
%% declarative formalism of \emph{array-based systems}.
%%Since their first introduction in~\cite{ijcar08,lmcs}, array-based systems have
%%been provided with various implementations of the standard backward
%%reachability algorithms (including more sophisticated variants and heuristics).
%Starting from its first version~\cite{mcmt}, \textsc{mcmt} was successfully
%applied to a variety of settings: cache coherence and mutual exclusions protocols~\cite{lmcs},
%timed~\cite{VERIFY} and fault-tolerant~\cite{jsat,disc} distributed systems, and imperative programs~\cite{atva,FI}. Interesting case studies
%concerned waiting time bounds synthesis in parameterized timed
%networks~\cite{nasa} and internet protocols~\cite{ifm}. Further related tools
%include \textsc{safari}~\cite{cav}, \textsc{asasp}~\cite{asasp}, and \textsc{Cubicle}~\cite{cubicle_cav}. The latter
%% ~\cite{Cubicle_FM,cubicle_fmcad,cubicle_cav,cubicle_ijcar}
%relies on a parallel architecture with further
%powerful extensions.
%%
%
%   
%Algorithm~\ref{alg1} describes the \emph{backward reachability algorithm}  for handling the safety problem for a RAS $\cS$.  An integral
%part of the algorithm is to compute preimages, i.e. the set of states that can reach the current states through a transition.
%The algorithm computes iterated preimages of the safety formula and applies to
%them quantifier elimination, until a fixpoint is reached or until a set
%intersecting the initial states (i.e., satisfying $\iota$) is found.
% %AG:dic
%The fixpoint is reached when the test in Line~2 returns \emph{unsat}, which means that the preimage of the set of the current states is included
%in the set of states reached by the backward search so far.
%
%The work principle of \textsc{mcmt} is rather simple: the tool generates the
%proof obligations arising from the safety and fixpoint tests in backward search
%(Lines~2-3 of Algorithm~\ref{alg1}) and passes them to the background
%SMT-solver (currently it is \textsc{Yices}~\cite{Dutertre}).  In practice, the
%situation is more complicated because SMT-solvers are quite efficient in
%handling satisfiability problems in combined theories at quantifier-free level,
%but may encounter difficulties with quantifiers. For this reason, \textsc{mcmt}
%implements modules for \emph{quantifier elimination} and \emph{quantifier
% instantiation}.  A \emph{specific module} for the quantifier elimination
%problems mentioned in Line~6 of Algorithm~\ref{alg1} has been added to
%Version~2.8 of \textsc{mcmt}.
%% (these seem to be new kinds of problems, with no available previous
%% implementation).

We have checked the encoding of the process  against five safe and five unsafe properties. The first property ascertains whether a job hiring case can actually reach the end point of the process, in turn witnessing soundness. The BPM\_SAFE1 property checks whether it is possible to have a situation where the \tname{Select Winner} task is $\senabled$ and the case variable $\cvar{result}$ indicates that the winner is not eligible.

 Table~\ref{tab:exp-results} shows the so-obtained, very encouraging results. Such initial results nicely complement those carried out on RAS in \cite{CGGMR18}, indicating that the approach is promising not just foundationally, but also in terms of tool support. These experiments, together with the ones reported in this paper, are available as part of the last distribution~2.8 of
\textsc{mcmt}.\footnote{\url{http://users.mat.unimi.it/users/ghilardi/mcmt/},
 subdirectory \texttt{/examples/dbdriven} of the distribution. The user manual
 contains a new section (pages 36--39) on how to encode \ras{s} in MCMT
 specifications.} Experiments were performed on a machine with Ubuntu~16.04, 2.6\,GHz Intel
Core~i7 and 16\,GB RAM.


\begin{table}[t!]
  \begin{tabularx}{\textwidth}{lXXlXX}
\footnotesize
    \textbf{Exp.}  & \textbf{Res.} & \textbf{Time (s)} & 
    \textbf{Exp.}  & \textbf{Res.} & \textbf{Time (s)} 
    \\\midrule
    BPM\_end\_process 
          & \unsafe   &  0.43
    \\
    BPM\_SAFE1  & \safe & 0.20 
    &
    BPM\_UNSAFE1 & \unsafe   & 0.18
    \\
    BPM\_SAFE2  & \safe & 5.85 
    &
    BPM\_UNSAFE2 & \unsafe & 1.17 
    \\
    BPM\_SAFE3 & \safe & 3.56 
    &
    BPM\_UNSAFE3 & \unsafe   & 4.45 
    \\
    BPM\_SAFE4  & \safe   & 0.03 
    &
    BPM\_UNSAFE4 & \unsafe & 1.43
    \\
    BPM\_SAFE5 &  \safe & 0.27 
    &
    BPM\_UNSAFE5 & \unsafe   & 1.14
    \\    
    \bottomrule
  \end{tabularx}
  \vspace{3pt}
\caption{Time spent by \mcmt to check different properties over the job hiring \dab. Names of experiments coincide with those of the \mcmt files from the Ancillary files of \url{arXiv:1905.12991}.}
\label{tab:exp-results}
\end{table}
 








\endinput


In order to verify safety properties over We implemented a prototype of the backward reachability algorithm for \ras{s} on top of the \textsc{mcmt} model checker for array-based systems.
% . \textsc{mcmt} manages verification in the infinite-state case by exploiting
% as its model-theoretic framework the declarative formalism of array-based
% systems.  This formalism allows for symbolic representation of transitions
% and sets of states using formulae, whereas the system dynamics is defined by
% manipulating second order variables (i.e., arrays).
%
% \textsc{mcmt}, in turn, is capable of verifying (safety) properties of a
% large class of infinite state systems which are specified using the
% declarative formalism of \emph{array-based systems}.
%Since their first introduction in~\cite{ijcar08,lmcs}, array-based systems have
%been provided with various implementations of the standard backward
%reachability algorithms (including more sophisticated variants and heuristics).
Starting from its first version~\cite{mcmt}, \textsc{mcmt} was successfully
applied to a variety of settings: cache coherence and mutual exclusions protocols~\cite{lmcs},
timed~\cite{VERIFY} and fault-tolerant~\cite{jsat,disc} distributed systems, and imperative programs~\cite{atva,FI}. Interesting case studies
concerned waiting time bounds synthesis in parameterized timed
networks~\cite{nasa} and internet protocols~\cite{ifm}. Further related tools
include \textsc{safari}~\cite{cav}, \textsc{asasp}~\cite{asasp}, and \textsc{Cubicle}~\cite{cubicle_cav}. The latter
% ~\cite{Cubicle_FM,cubicle_fmcad,cubicle_cav,cubicle_ijcar}
relies on a parallel architecture with further
powerful extensions.
%
The work principle of \textsc{mcmt} is rather simple: the tool generates the
proof obligations arising from the safety and fixpoint tests in backward search
(Lines~2-3 of Algorithm~\ref{alg1}) and passes them to the background
SMT-solver (currently it is \textsc{Yices}~\cite{Dutertre}).  In practice, the
situation is more complicated because SMT-solvers are quite efficient in
handling satisfiability problems in combined theories at quantifier-free level,
but may encounter difficulties with quantifiers. For this reason, \textsc{mcmt}
implements modules for \emph{quantifier elimination} and \emph{quantifier
 instantiation}.  A \emph{specific module} for the quantifier elimination
problems mentioned in Line~6 of Algorithm~\ref{alg1} has been added to
Version~2.8 of \textsc{mcmt}.
% (these seem to be new kinds of problems, with no available previous
% implementation).

We produced a benchmark consisting of eight realistic business process examples
and ran it in \textsc{mcmt} (detailed explanations and results are given in
Appendix~\ref{app_experiments}). The examples are partially made by hand and
partially obtained from those supplied in~\cite{verifas}. A thorough comparison
with \textsc{Verifas}~\cite{verifas} is matter of future work, and is
non-trivial for a variety of reasons.  In particular, the two systems tackle
incomparable verification problems: on the one hand, we deal with safety
problems, whereas \textsc{Verifas} handles more general LTL-FO properties.  On
the other hand, we tackle features not available in \textsc{Verifas}, like bulk
updates and comparisons between artifact tuples.
%
Moreover, the two verifiers implement completely different state space
construction strategies: \textsc{mcmt} is based on backward reachability and
makes use of declarative techniques that rely on decision procedures, while
\textsc{Verifas} employs forward search via VASS encoding.
%
% for the following reasons:
% \begin{inparaenum}[\itshape (i)]
% \item We deal with safety problems, whereas \textsc{Verifas} handles more
%   general LTL-FO properties. At the same time, our setting is more expressive
%   (e.g., we cover ``bulk'' updates).
% \item \textsc{mcmt} is based on backward reachability, while \textsc{Verifas}
%   employs forward search via VASS encoding; hence, the state space in the two
%   approaches may differ extensively depending on the given system and
%   property.
%   % two complementary methods
% \item \textsc{mcmt} takes as input user-defined safety properties,
%   %   and this can be also applied to our benchmark. In turn,
%   while \textsc{Verifas} works on predefined LTL-FO templates, automatically
%   instantiated based on syntactic criteria.\item The tools use different
%   input specification languages.
%   %   that complicates their experimental comparison.
% \end{inparaenum}

The benchmark is available as part of the last distribution~2.8 of
\textsc{mcmt}.\footnote{\url{http://users.mat.unimi.it/users/ghilardi/mcmt/},
 subdirectory \texttt{/examples/dbdriven} of the distribution. The user manual
 contains a new section (pages 36--39) on how to encode \ras{s} in MCMT
 specifications.}  Table~\ref{tab:exp-results} shows the very encouraging
results (the first row tackles Example~\ref{ex:hr-prop}). While a systematic
evaluation is out of scope, \textsc{mcmt} effectively handles the benchmark
with a comparable performance shown in other, well-studied systems, with
verification times below 1s in most cases.

% In fact, all of the cases presented in our benchmark are discharged quite
% quickly. In particular, more than 90\% are resolved in less than one second,
% while the most challenging for \textsc{mcmt} case took only 4.11 seconds.
% (in less than one second), whereas more sensible timings arise in case of
% significantly built up problems.

% \todo[inline]{One can see, for example, that the job hiring \ras has been
% proved by MCMT to be safe w.r.t. the property defined in
% Example~\ref{ex:hr-prop}. The details about the successfully completed
% verification task can be seen in the first row of Table~\ref{}: the tool
% constructed a tree with N nodes and a depth of M, and returned \safe{} in K
% seconds. \textbf{REFERENCE COLUMNS}}
